Seeing is Believing: Vision-driven Non-crash Functional Bug Detection for Mobile Apps

Mobile app GUI (Graphical User Interface) pages now contain rich visual information, with the visual semantics of each page helping users understand the application logic. However, these complex visual and functional logic present new challenges to software testing. Existing automated GUI testing methods, constrained by the lack of reliable testing oracles, are limited to detecting crash bugs with obvious abnormal signals. Consequently, many non-crash functional bugs, ranging from unexpected behaviors to logical errors, often evade detection by current techniques. While these non-crash functional bugs can exhibit visual cues that serve as potential testing oracles, they often entail a sequence of screenshots, and detecting them necessitates an understanding of the operational logic among GUI page transitions, which is challenging traditional techniques. Considering the remarkable performance of Multimodal Large Language Models (MLLM) in visual and language understanding, this paper proposes Trident, a novel vision-driven, multi-agent collaborative automated GUI testing approach for detecting non-crash functional bugs. It comprises three agents: Explorer, Monitor, and Detector, to guide the exploration, oversee the testing progress, and spot issues. We also address several challenges, i.e., align visual and textual information for MLLM input, achieve functionality-oriented exploration, and infer test oracles for non-crash bugs, to enhance the performance of functionality bug detection. We evaluate Trident on 590 non-crash bugs and compare it with 12 baselines, it can achieve more than 14%-112% and 108%-147% boost in average recall and precision compared with the best baseline. The ablation study further proves the contribution of each module. Moreover, Trident identifies 43 new bugs on Google Play, of which 31 have been fixed.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> figure/Pilot-study.tex <==
\begin{figure}[!thb]
\vspace{-0.1in}
\centering
\includegraphics[width=5.9cm]{figure/Pilot-study.png}
\caption{The categories of non-crash functional bugs}
% \chen{For some components, you can make it shorter by using some abbreviation e.g., feedback missing, nav\&linking errors, setting\&config failures, media no response...}}
% \jie{comment}}
%都是百分号，只有media那里，是12
\label{fig:Pilot-study}
\vspace{-0.15in}
\end{figure}

==> figure/annotation-example.tex <==
\begin{figure}
\centering
\vspace{-0.1in}
\includegraphics[width=8.3cm]{figure/annotation-example.png}
\caption{Example of annotation in our {\tool}\jie{comment}
%如果后面有时间，这个可以搞成有三种颜色的，现在就两种感觉不是特别容易观察到。但这个问题不大，后面有时间再说。
} 
\label{fig:annotation-example}
\vspace{-0.1in}
\end{figure}

==> figure/detect-prompt.tex <==
\begin{figure}[htb]
\centering
\vspace{0.1in}
\includegraphics[width=8.3cm]{figure/Detect-prompt.png}
\caption{Example of bug detection prompt}
% \chen{1. some typos in the bug detect part: bug detection, that transits, expected oracle --> expectation, no-crash --> any. 2.Make the screenshot larger, move the text to the image caption. 3. This figure should be behind the Figure 7.}}
% \jie{comment}
%、figure 5里面examples那里，还说了image，这里要说image吗
%bug detection 首字母的B 大写。defects，都统一用bugs吧 就在bug detect的第二行的最后，还有最后一行。最后一个interface，改成page？
% }
\label{fig:detect-prompt}
\vspace{-0.15in}
\end{figure}

==> figure/explore-prompt.tex <==
\begin{figure}[htb]
\centering
\includegraphics[width=8.5cm]{figure/explore-prompt.png}
\caption{Example of explorer prompt}
% \jie{comment}
%querying 那两个感觉不应该是optional，应该是二选一，如果optional都不选，那就没有action了，可能也不是二选一，因为有些时候两个都有，要不就把 input 改成 optional，或者就都不标了？
% } 
% \chen{1)Should we add "Optional" to the testing feedback? What if there is no mistake? 2) try to make the screenshot larger, while putting the text to the figure caption, rather than on the left to the image.}}
% \jie{comment}
%gui text info 后面那块，是个句号吗，还是还可能有内容，用省略号
%explored function那里，visit number to（改成of）
%history那块，four steps那里，the “”step“”是啥内容？the bounding是啥内容？
%querying 那里，widget id吧，不应该是number。which numbered widget也很奇怪。give the widget id that need to take action?
%testing feedback 也是，用id
%紫色那个，action & feedback & question，不用question了吧
% }
% \jie{should annotate where are the detailed figures}}
\label{fig:explore-prompt}
\vspace{-0.15in}
\end{figure}

==> figure/overview-2.tex <==
\begin{figure}[htb]
\centering
\includegraphics[width=8.6cm]{figure/overview-2.png}
\caption{overview-2}
\label{fig:overview-2}
\vspace{-0.1in}
\end{figure}

==> figure/test-seq-example.tex <==
\begin{figure*}[t]
\centering
\vspace{-0.15in}
\includegraphics[width=18.0cm]{figure/test-seq-example.png}
% \vspace{-0.05in}
\caption{Example of sequence segmentation and bugs detected by {\tool}}
% \chen{Is there any example that we can see clearly two or more full communities are separated?} } 
\label{fig:test-seq-example}
\vspace{-0.15in}
\end{figure*}


==> tab/RQ1-different-setting.tex <==
\begin{table}[h]
\vspace{0.1in}
\renewcommand\arraystretch{1.1} 
\caption{Result of state transition passing rate.(RQ1)}
\vspace{-0.05in}
\label{tab:RQ1-different-setting}
\centering
\footnotesize
\begin{tabular}{p{1.6cm}<{\centering} | p{0.8cm}<{\centering} | p{0.6cm}<{\centering} | p{0.6cm}<{\centering} | p{0.8cm}<{\centering} | p{0.8cm}<{\centering} | p{0.6cm}<{\centering}}
% \hline
\toprule
\textbf{Method} & \textbf{Person} & \textbf{Geo} & \textbf{Num} & \textbf{Search} & \textbf{Comm} & \textbf{All}\\ 
\midrule
\multicolumn{7}{c}{\textbf{Without context information}}\\
\midrule
QTypist (-ct) & 0.47  & 0.32  & 0.37  & 0.36  & 0.72  & 0.44 \\ 
\midrule
\multicolumn{7}{c}{\textbf{Prompt tuning data setting}}\\
\midrule
Zero-shot & 0.58  & 0.53  & 0.42  & 0.52  & 0.78  & 0.56 \\ 
25\% data & 0.68  & 0.68  & 0.63  & 0.60  & 0.83  & 0.68 \\ 
50\% data & 0.74  & 0.79  & 0.74  & 0.72  & 0.89  & 0.77 \\ 
75\% data & 0.79  & 0.84  & 0.79  & 0.80  & 0.89  & 0.82 \\
\textbf{QTypist} & \textbf{0.84}  & \textbf{0.89}  & \textbf{0.84}  & \textbf{0.88}  & \textbf{0.89}  & \textbf{0.87} \\
\bottomrule
\end{tabular}
\vspace{0.05in}
\vspace{-0.1in}
\end{table}




==> tab/RQ1-result-inter.tex <==
\begin{table}[h]
% \vspace{-0.05in}
\renewcommand\arraystretch{0.95} 
\caption{Result of inter-page bug detection. (RQ1)}
\vspace{-0.05in}
\label{tab:RQ1-result-inter}
\centering
\footnotesize
\begin{tabular}{p{1.4cm}<{\centering} | p{0.6cm}<{\centering} | p{0.6cm}<{\centering} | p{0.6cm}<{\centering} | p{0.6cm}<{\centering} | p{0.8cm}<{\centering} | p{0.6cm}<{\centering}}
% \hline
\toprule
\multirow{2}*{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Baseline data}} & \multicolumn{2}{c|}{\textbf{GitHub data}} & \multicolumn{2}{c}{\textbf{Bug injection data}} \cr 
& \textbf{P} & \textbf{R} & \textbf{P} & \textbf{R} & \textbf{P} & \textbf{R}\\ 
% \hline
\midrule
Genie & 0.38  & 0.27  & 0.27  & 0.15  & 0.18  & 0.30 \\ 
Odin & 0.31  & 0.18  & 0.33  & 0.21 & 0.23  & 0.37 \\ 
\midrule
iFixdataloss & 0.11  & 0.04  & 0.11  & 0.08  & 0.07  & 0.08 \\ 
SetDroid  & 0.13  & 0.21  & 0.19  & 0.23  & 0.18  & 0.13 \\ 
\midrule
Lint & 0.09  & 0.13  & 0.08  & 0.05  & 0.03  & 0.15 \\ 
LiveDroid  & 0.05  & 0.13  & 0.13  & 0.12  & 0.12  & 0.21 \\ 
\midrule
\textbf{{\tool}} & \textbf{0.70}  & \textbf{0.73}  & \textbf{0.79 } &\textbf{ 0.86 } & \textbf{0.75}  & \textbf{0.71} \\ 
\bottomrule
\end{tabular}
\vspace{0.05in}
\begin{tablenotes}
\footnotesize
\item \textbf{\textit{Notes:}} ``P'' is the Precision, ``R'' is the Recall.
\end{tablenotes}
\vspace{-0.1in}
\end{table}


==> tab/RQ1-result-intra.tex <==
\begin{table}[h]
% \vspace{-0.05in}
\renewcommand\arraystretch{0.95} 
\caption{Result of intra-page bug detection. (RQ1)}
\vspace{-0.05in}
\label{tab:RQ1-result-intra}
\centering
\footnotesize
\begin{tabular}{p{1.4cm}<{\centering} | p{0.6cm}<{\centering} | p{0.6cm}<{\centering} | p{0.6cm}<{\centering} | p{0.6cm}<{\centering} | p{0.8cm}<{\centering} | p{0.6cm}<{\centering}}
\toprule
\multirow{2}*{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Baseline data}} & \multicolumn{2}{c|}{\textbf{GitHub data}} & \multicolumn{2}{c}{\textbf{Bug injection data}} \cr 
& \textbf{P} & \textbf{R} & \textbf{P} & \textbf{R} & \textbf{P} & \textbf{R}\\ 
% \hline
\midrule
OwlEyes & 0.43  & 0.29  & 0.37  & 0.23  & 0.39  & 0.30 \\ 
NightHawk & 0.51  & 0.57  & 0.49  & 0.53  & 0.53  & 0.37 \\ 
DiffDroid & 0.11  & 0.04  & 0.08  & 0.05  & 0.03  & 0.11 \\ 
dVermin  & 0.23  & 0.33  & 0.15  & 0.25  & 0.35  & 0.29 \\ 
\midrule
{\tool} & 0.78  & 0.88  & 0.83  & 0.81  & 0.85  & 0.87 \\ 
\bottomrule
\end{tabular}
\vspace{0.05in}
\begin{tablenotes}
\footnotesize
\item \textbf{\textit{Notes:}} ``P'' is the Precision, ``R'' is the Recall.
\end{tablenotes}
\vspace{-0.1in}
\end{table}



==> tab/explorer-rule.tex <==
\begin{table*}
% \vspace{-0.1in}
\renewcommand\arraystretch{0.95} 
\caption{The example of linguistic patterns of prompts and generation rules.}
% \vspace{-0.1in}
\label{tab:explorer-rule}
\centering
\footnotesize
% \scriptsize
% \begin{center}
\begin{tabular}{p{0.2cm}<{\centering} | p{2.2cm} | p{6.3cm}<{} | p{7.9cm}<{}}
\toprule
\textbf{Id} & \textbf{Pattern type} & \textbf{Sample of linguistic patterns/rules} & \textbf{Instantiation}\\
\midrule
\multicolumn{4}{c}{\textbf{GUI information patterns: \hlr{\textit{GUIInfo}}}} \\ 
% \rowcolor{red!10}
\midrule
\rowcolor{red!10}
1 & App \& page information & Please be a tester to test [\textit{AppName}] App. It has the following activities, including [\textit{Activities}]. The current tested page is [\textit{ActivityName}]. & 
Please be a tester to test the ``American Airlines'' App. It has the following activities, including ``Main'', ``SearchFlight'', ``Setting'', ... . The current tested page is ``SearchFlight''. \\
\rowcolor{red!10}
\midrule
2 & Legend of current & \multicolumn{2}{l}{On the right side of the image is the currently tested page. We label the actionable widgets in the first column of each row in} \\
\rowcolor{red!10}
 &  GUI screenshots &  \multicolumn{2}{l}{order from left to right, please infer the other number in each row. We also label the types of actionable widgets according to}\\
\rowcolor{red!10}
 &  & \multicolumn{2}{l}{the rules, with red as ``click'', blue as ``input'', purple as ``long click'', pink as ``check'', and yellow as ``scroll''.}\\
\midrule
\multicolumn{4}{c}{\textbf{Function-based history patterns: \hlb{\textit{History}}}} \\ 
\midrule
\rowcolor{blue!10}
3 & Explored functions & Up to now, the tested functions and the visit number to each function are as follows: [\textit{Function Name}] + [\textit{Visits Time}], [\textit{Function Name}] + [\textit{Visits Time}] ... & Up to now, the tested functions and the visit number to each function are as follows: ``Function1: Main. Visits: 4.'', ``Function2: Search flight number. Visits: 2.'', ... \\
\midrule
\rowcolor{blue!10}
4 & Legend of recently & \multicolumn{2}{l}{On the left side of the image are the screenshots from the last 4 steps with the labeled action widget. Each screenshot is label} \\
\rowcolor{blue!10}
 & tested screenshots & \multicolumn{2}{l}{-ed with the function name of the tested page.}\\
\midrule
\multicolumn{4}{c}{\textbf{Action \& feedback \& function question patterns: \hlg{\textit{OperationQuestion}}}} \\ 
\midrule
\rowcolor{green!10}
5 & Querying Function & Function question + [\textit{Output Template}] & Please make a judgment based on the GUI information on the page. What is the function currently being tested? Are we testing a new function? ([\textit{FunctionName}]  + [\textit{Status}])  \\ 
\midrule
\rowcolor{green!10}
6 & Querying general action & Action question + [\textit{Output Template}] & Which numbered widget? What actions are needed? What is the textual description of the widget? ([\textit{Widget number}] + [\textit{Action}][click / long-click / check / scroll] + [\textit{Widget text}] ) \\
\midrule
 \rowcolor{green!10}
7 & Querying text input & Input operation question + [\textit{Output Template}]& Please give the widget number, generate the input text, and the action after input. ([\textit{Widget number}]+[\textit{Input Content}], ...) and provided ([\textit{Widget number}] + [\textit{Action}[click]] + [\textit{Widget text}]) \\
\midrule
 \rowcolor{green!10}
8 & Testing feedback & Feedback question & The widget number matches the widget text incorrectly. Please provide the correct widget number again.
 \\ 
\bottomrule
\toprule
\multicolumn{4}{c}{\textbf{Prompt generation rules}}\\
\midrule
1 & \multicolumn{3}{l}{\textbf{Test Prompt:} \hlr{\textit{GUIInfo}[1,2]} + \hlb{\textit{History}[3,4]} +\hlg{\textit{OperationQuestion}[5,6/7]}}  \\
\midrule
2 & \multicolumn{3}{l}{\textbf{Feedback Prompt:} Sorry,  \hlg{[\textit{OperationQuestion}][8]} + \hlr{\textit{GUIInfo}[1,2]} +  \hlb{\textit{History}[3,4]} +\hlg{\textit{OperationQuestion}[6/7]}} \\
\bottomrule
\end{tabular}
\begin{tablenotes}
% \footnotesize
\scriptsize
\item \textbf{\textit{Notes:}} ``[1,2, ..., 6]'' means the id of each pattern. If there is ``EditText'' on the page, {\tool} selects ``Querying text input'' pattern. For the other widgets, {\tool} selects ``Querying general action'' pattern.
\end{tablenotes}
% \end{center}
\vspace{-0.1in}
% \vspace{-0.15in}
\end{table*}

